Introducing and Interfacing with Cybersecurity -- A Cards Approach

Cybersecurity is an important topic which is often viewed as one that is inaccessible due to steep learning curves and a perceived requirement of needing specialist knowledge. With a constantly changing threat landscape, practical solutions such as best-practices are employed, but the number of critical cybersecurity-related incidents remains high. To address these concerns, the National Cyber Security Centre published a Cybersecurity Body of Knowledge (CyBOK) to provide a comprehensive information base used to advise and underpin cybersecurity learning. Unfortunately, CyBOK contains over 1000 pages of in-depth material and may not be easy to navigate for novice individuals. Furthermore, it does not allow for easy expression of various cybersecurity scenarios that such individuals may be exposed to. As a solution to these two issues, we propose the use of a playing cards format to provide introductory cybersecurity knowledge that supports learning and discussion, using CyBOK as the foundation for the technical content. Upon evaluation in two user studies, we found that 80% of the participants agreed the cards provided them with introductory knowledge of cybersecurity topics, and 70% agreed the cards provided an interface for discussing topics and enabled them to make links between attacks, vulnerabilities and defences.

==> sections/background.tex <==
%-------------------------------------------------------------------------------
\section{Background}
\label{sec:background}
%-------------------------------------------------------------------------------

The need for practical and easy-to-learn cybersecurity learning material is a constant problem which stems from
the evolving nature of vulnerabilities, threats, attacks and defences as the number of connected
users and devices scales. In recent years, the number of critical cybersecurity
incidents have increased significantly, correlating with increasing numbers of
online users during the Covid-19 pandemic, for example, as well as an increase in the
adoption of various connected computer systems in day-to-day activities. Among these
incidents, research shows that around 95\% of cybersecurity breaches occur as a
result of human error~\cite{wef2020} and that organisations lack the sophistication, interest and/or
knowledge to handle these threats~\cite{ciscoreport2020,sophos2021}.

It has been shown that those in cybersecurity careers require a set of skills, involving the
abilities to carry out various tasks at any time in non-traditional environments, and adapt to
the dynamic nature of these environments~\cite{niccs2015}. In the domain of software engineering,
basic cybersecurity training such as password best-practices and multi-factor authentication are
employed for individuals to conform to, with the aim of alleviating concerns and mitigating the
potential for liabilities that arise as a result of cybersecurity-related
incidents~\cite{walters2011assessing,alotaibi2018review,sarginson2020securing}. In the domain of
software engineering, for example, simply employing these best practices are not enough as there are
additional requirements of ensuring developers code securely. It has been identified that a large
number of Android applications contain security-related code snippets copied and pasted from Stack Overflow,
of which nearly 98\% contained at least one insecure code snippet~\cite{fischer2017stack}. This was also shown to
be true upon scanning open-source projects in different programming languages~\cite{hong2021dicos}. The
value of security information depends strongly on its source~\cite{rader2015identifying} and reputable information
sources are only useful, so long as they are well-understood and perceived as
actionable~\cite{thomas2019educational,redmiles2020comprehensive}. While sites such as StackOverflow are reputable
for providing actionable solutions to problems that are asked on them, it is clear that the security of solutions
are not well understood, either by the responder or those who interpret them. Thus, are software developers
truly {\em informed} to the extent they actually understand why certain security measures are put in place, and the
true impact of not adhering to best-practices and secure coding. For novice individuals, such as those who write
and/or deploy software code without formal software engineering training, cybersecurity may appear intimidating or
confusing, and may require more specialist knowledge or guidance to promote adequate learning and understanding.

To address this, various curricula guidelines and knowledge frameworks have been developed for
cybersecurity, covering a range of fundamental topics ranging from software and hardware security, to networks and
cyber-physical systems. The Joint Task Force (JTF) on Cybersecurity Education propose a draft of
curricular guidance on cybersecurity to support educational efforts~\cite{bishop2017cybersecurity}.
They design a framework model for a body of knowledge that covers six knowledge areas which
several concepts span over, targeting specific disciplines and application areas which pertain to
the demographic of cybersecurity professionals. The National Initiative for Cybersecurity Education
(NICE)~\cite{newhouse2017national} is a cybersecurity workforce framework which aims to provide
a foundation for describing and sharing information about knowledge, skills and abilities in
cybersecurity to strengthen an organisation's cybersecurity. The NCSC propose a Certified Master's
Program that defines several pathways to address knowledge and skill gaps in cybersecurity education,
which describe what topics must be covered and to what depth~\cite{ncscmsc}. While all these frameworks
tend to agree on key cybersecurity topics that must be understood, they only promote greater
emphasis on a subset of topics. For example, NICE covers a wide range of key topics but gaps exist
such as with topics related to cyber-physical systems and human factors, and the NCSC Certified
Master's Program guidelines do not put much emphasis on important topics such as software security, but
in contrast with others place emphasis on attacks and defences. The CyBOK knowledge base is decomposed
into 21 knowledge areas (KAs) (as of version 1.1), each introduced by a reference document and a set
of topics presented as a branch of the overall {\em Knowledge Tree}
(Figure~\ref{fig:cybokfulltree})~\cite{cybokwebsite}. Each of these knowledge areas are organised into a hierarchy
of 5 categories. It has been shown that, in comparison with other knowledge frameworks, CyBOK covers a wider range
of knowledge areas and does not have gaps that are present with other frameworks~\cite{hallett2018mirror}.
% Ultimately, the goal of these bodies of knowledge is to provide
% both a taxonomy of various cybersecurity topics and references which can be used to facilitate the development
% and review of cybersecurity curricula and learning materials.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{img/cybokfulltree.pdf}
    \caption{\centering Partial View of CyBOK 1.1 Knowledge Tree~\cite{cybokwebmobile}}
    \label{fig:cybokfulltree}
\end{figure*}

For each KA in CyBOK, there is a collection of reports that form an encyclopedic collection of
knowledge of key concepts backed up by state-of-the-art academic literature.
The key concepts that are covered in each KA are known as {\em Topics}. Some Topics
decomposed further into a set of more specialised subjects ({\em Sub-Topics}).
%For example,
%{\em "SQL Injection"} is a portrayed as a {\em Sub-Topic} of
%{\em "Injection Vulnerabilities"} (Figure~\ref{fig:cyboktree}).
At its core, the CyBOK Knowledge Tree aims to provide a systematic approach to traversing an exhaustive list of various
cybersecurity topics and mapping to the tree facilitates links to other resources.

%\begin{figure}[h]
%    \centering
%    \includegraphics[width=\linewidth]{img/cyboktree.pdf}
%    \caption{\centering Partial View of CyBOK 1.1 Knowledge Tree~\cite{cybokwebmobile}}
%    \label{fig:cyboktree}
%\end{figure}

While CyBOK facilitates a body of knowledge which attributes to the production of material for cybersecurity
education and professional training, there are some weaknesses which may render it an inaccessible resource to
more novice individuals such as those in the domain of software engineering who write or deploy code with no formal
software engineering training. First, the links between meaning and relationships among topics and sub-topics
vary across the entire Knowledge Tree, which prevents easy expression of various cybersecurity
scenarios. Second, the material across the CyBOK knowledge base and its indexing structure is not easy to traverse
for novice users. Gonzalez et al.~\cite{gonzalez2022exploring} show that it would be difficult for novice individuals
to infer the links between various topics, given that some follow either a single predominant theme or span several
topics themselves. Ultimately, to support novice users as well as those more experienced, key cybersecurity knowledge
provided by knowledgebases such as CyBOK require adequate presentation that can faciliate independent learning whilst
also providing a suitable interface for discussion of various cybersecurity scenarios to make the links between meaning
and relationships among topics.

Aside from knowledge frameworks, such as CyBOK, cybersecurity information and how it
is perceived and understood has also been presented in other ways.
Capture the Flag (CTF) activities provide a series of competitive exercises used to find
vulnerabilities in computer systems and applications, and have shown to be a valuable
learning tool~\cite{trickel2017shell,cybokctf,swann2021open}. Thomas et
al.~\cite{thomas2019educational} propose the use of a collectible
card game (CCG) as a means of teaching cybersecurity to high school students, given the benefits of
prevalence culturally to all age groups (familiarity) and encouraging the understanding
of competitive strategy and mistake-making as a way of learning~\cite{turkay2012collectible}.
Anvik et al.~\cite{anvik2019program} propose the use of a web-based card game for learning
programming and cybersecurity concepts, using simple vocabulary to create ubiquitous learning
experiences. Denning et al.~\cite{denning2013control} propose the use of a tabletop card game,
Control-Alt-Hack, with the aim of providing awareness training for cybersecurity,
arguing that playing card games can provide a reachable foundation for providing digestible
cybersecurity information to large audiences. However, while these gamified approaches show
various levels of success, there are limitations. For example, card game approaches such as
Control-Alt-Hack~\cite{denning2013control} do not cover a broad range of key cybersecurity topics,
such as those identified by knowledge frameworks such as CyBOK, and do not adequately highlight
the links between vulnerabilities, attacks and defences. Specifically, attacks are typically
highlighted first, which does not help users understand how attacks present themselves (opportunistic
vulnerability targeting) and how to protect against them. While CTF activities, for example, are
beneficial in this aspect~\cite{swann2021open,trickel2017shell}, a key disadvantage pertains to
novice users wherein competitions rely on technical expertise and the ability to traverse computer systems
using various command-line tools and other bespoke applications~\cite{ford2017capture}, or requiring (at
a minimum) a basic understanding of cybersecurity concepts in order to progress in finding vulnerabilities~\cite{mcdaniel2016capture}.

==> sections/cards.tex <==
%-------------------------------------------------------------------------------
\section{Cybersecurity Cards (Version 1)}
\label{sec:cards}
%-------------------------------------------------------------------------------

The weaknesses of existing solutions we have identified regarding the limitations of accessibility,
steep learning curves and a perceived requirement of specialist knowledge/expertise
must be ameliorated by a new solution that provides an answer to the following
research questions. Specifically, can the new solution:

\begin{questions}[leftmargin=*,align=left]%[itemindent=0.18in]
    \item Provide introductory cybersecurity knowledge to novice users?
    \item Provide material for expressing interpretation and documentation of key cybersecurity topics, which can support independent learning and self-efficacy?
    \item Act as an index for the CyBOK knowledge base which provides an interface for discussion on key cybersecurity topics?
    \item Provide links between key cybersecurity topics, allowing the generation of concepts which can capture various cybersecurity scenarios?
\end{questions}
% \end{enumerate}

To answer these research questions, we propose a novel approach to represent key cybersecurity
knowledge, utilising specially designed playing cards. In recent years, it has
been shown that specially designed cards used as a tool for education attributes to positive outcomes in the space of
learning, attitudes and critical thinking skills~\cite{kordaki2016computer,kordaki2017digital}. With a large portion
of the general population familiar with card-based games, it is clear that a playing card format is a good medium,
both physically and digitally, with relatively intuitive logic if they are designed well. A subset of the cards
we propose in this section have been made available for viewing and can be found
online\footnote{\url{https://anonymous.4open.science/r/cybersecurity_cards-9F00/}}. The full set of cards will be made
publicly available under the CC BY-NC-SA Creative Commons license after the research project ends in January 2024.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\linewidth]{img/cards-v1.pdf}
    \caption{\centering Organisation and Design of Cybersecurity Cards (Version 1)}
    \label{fig:carddesign}
\end{figure}


\subsection{Focus of Knowledge}

In order to establish a good grounding for an evaluation of a card-based solution to address the proposed research
questions, an important factor is to determine what information the card aims to represent. In this work, we leverage
the information found in the CyBOK knowledge base and produce the cybersecurity cards to address the limitations of
the knowledge base. Specifically, the focus of knowledge we chose to take is in the domain of software engineering,
given recent increases in threats pertaining to this domain~\cite{saxena2020impact,pranggono2021covid} and the
observation of finding people with skills in secure coding reported as the most difficult task~\cite{willetts2014cyber}.

The topics that fall within the scope of the focus of knowledge in this work were derived from a filtering and
selection procedure, where the CyBOK knowledge tree was traversed from Knowledge Areas to Topics. Given that not all
KAs in CyBOK are related to the domain of software engineering, we selected topics that related to this theme.
As highlighted in Figure~\ref{fig:cybokfulltree}, we chose the following knowledge trees to traverse:
{\em Human Factors}, {\em Malware \& Attack Technologies}, {\em Software Security}, {\em Web \& Mobile Security} and the
{\em Secure Software Lifecycle}. For each KA, we follow each branch of the tree to the leaf nodes. For each of the
leaves, we pick up the topic and provide a better description of that name to create the first version of the card. If
there are duplicates or highly similar cards, these are merged together. Any leaves that fall within Topics that, for
example, may not follow a single predominant theme and do not relate to the selected focus of knowledge are cut. For
example, {\em Software \& Platform Security} category are disdrectly related to the scope of this work whereas others are
not, such as {\em Forensics} which involves identifying and analysing data to support legal proceedings. This process
was carried out by two academic researchers in cybersecurity who decided on the final first set of cards in consensus.

%\begin{table*}
%  % \begin{center}
%    \begin{tabularx}{\linewidth}{m{0.1\linewidth}m{0.125\linewidth}cm{0.60\linewidth}}
%      \toprule
%      \textbf{Class} & \textbf{General Card} & \textbf{Symbol} & \textbf{Description} \\
%      \midrule
%      \multirow{3}{\linewidth}{Vulnerability} &
%                      Environment & \includegraphics[valign=c,width=0.035\linewidth]{img/EnvironmentV Icon.png} & Badly configured execution environment can leak out information and allow malicious users to attack the services above it \\ &
%                      Code & \includegraphics[valign=c,width=0.035\linewidth]{img/CodeV Icon.png} & Badly written code can allow malicious users to alter the functionality, getting extra information or crashing the services \\ &
%                      Human & \includegraphics[valign=c,width=0.035\linewidth]{img/HumanV Icon.png} & Bad practice by careless user or bad defence against corrupted internal user can allow malicious users to gain insider knowledge or privilege through social and psychological skills \\
%      \midrule
%      \multirow{8}{\linewidth}{Attack} &
%                      Memory & \includegraphics[valign=c,width=0.035\linewidth]{img/Memory Icon.png} & Targets the memory and storage of modern computers or hides its existence in the memory in fileless status \\ &
%                      Injection & \includegraphics[valign=c,width=0.035\linewidth]{img/Injection Icon.png} & Alters original functionality or adds extra executions on the original services \\ &
%                      Race Condition & \includegraphics[valign=c,width=0.035\linewidth]{img/Race Condition Icon.png} & Abuses race conditions to get undesired output \\ &
%                      Side Channel & \includegraphics[valign=c,width=0.035\linewidth]{img/Side Channel Icon.png} & Studies the outside behaviour to get information of the execution paths, resources used or other hidden details for further attack \\ &
%                      Authentication & \includegraphics[valign=c,width=0.035\linewidth]{img/Authentication Icon.png} & Breaks normal authentication process to perform actions with fake or privileged identity \\ &
%                      Web & \includegraphics[valign=c,width=0.035\linewidth]{img/Web Icon.png} & Targets web services or redirects attacks towards other users by abusing web services \\ &
%                      Human Factor & \includegraphics[valign=c,width=0.035\linewidth]{img/Human Factor Icon.png} & Trick users to providing information of some privileged access or resources. Also refers to insiders purposely doing damage to internal services \\ &
%                      System & \includegraphics[valign=c,width=0.035\linewidth]{img/SystemA Icon.png} & Spreads through computers without user notice in the form of malicious software or bundle of attack commands that target basic system functionality and settings \\
%      \midrule
%      \multirow{4}{\linewidth}{Defence} &
%                      Detection & \includegraphics[valign=c,width=0.035\linewidth]{img/Detection Icon.png} & Detect and notify the administrator about possible attacks happening. Allows live defence and tracing for forensic purposes \\ &
%                      Mitigation & \includegraphics[valign=c,width=0.035\linewidth]{img/Mitigation Icon.png} & Decrease the possibility or effect of certain attacks \\ &
%                      Prevention & \includegraphics[valign=c,width=0.035\linewidth]{img/Prevention Icon.png} & Stop some types of attack \\ &
%                      Education & \includegraphics[valign=c,width=0.035\linewidth]{img/Education Icon.png} & Provide education to users to decrease the chance of being targeted \\
%      \bottomrule
%    \end{tabularx}
%    \caption{\centering List of General Cards (Version 1)}
%    \label{table:basecards}
%  % \end{center}
%\end{table*}


\subsection{Design and Structure}

The playing cards format is easy to handle in both a physical or digital medium~\cite{altice2014playing} and are
designed to be handled individually or combined into a set of cards (known as a {\em deck}). The deck of cards is first
split into three distinct classes: \textbf{Vulnerability}, \textbf{Attack} and \textbf{Defence}, following suit from
common threat modelling approaches and security catalogues that encompass the vulnerability-attack-defence
dichotomy~\cite{kordy2014attack,ferro2021human,tatam2021review,cve,martin2011cwe}. Within each of these classes, the
deck is further split into {\em \textbf{General}} and {\em \textbf{Detailed}} cards (Figure~\ref{fig:carddesign}).
General cards represent a type of one of the classes (e.g. {\em Code}), while Detailed cards provide lower-level,
concrete examples that relate to the General card.

In terms of design (Figure~\ref{fig:carddesign}), attack and vulnerability cards are encased in a square border, with
attack cards filled with a solid red colour while vulnerability cards a signalled with a diagonal line to separate
white from red. The defence cards resemble an octogonal shape (akin to a shield) which has a white fill colour. The
diagonal separation of white and red in vulnerability cards aims to highlight vulnerabilities being the center of
the attack-defence dichotomy.

General cards in the deck include: a title representing the KA topic; a type represented
by a symbol (see \circled{1}); and a description related to the topic it represents. Detailed cards are assigned a
unique identifier in the form {\em $a\_Bi$} in the top right corner \circled{2}, where $a$ refers to the class of the
Detailed card, $B$ referring to the first letter of the General card it is categorised under and $i$ acting as an
index number in the set of $N$ Detailed cards for the category $B$. The symbol for the Detailed card's category is
made opaque in the center of the card, behind the description of the Detailed card. Attack cards also contain a
description of the impact of the attack. Defence cards contain a target symbol to help further identify the
vulnerability it aims to protect against attacks. Vulnerability cards also describe an attack vector with associated
attack card identifiers, as well as the consequence of the vulnerability with associated defence card identifiers
\circled{3}. In total, there are 124 cards in the deck which is composed of 30 vulnerability cards, 32 attack cards and
47 defence cards, each of which are categorised under one of the 15 General cards.

\subsubsection{Relationships Between Cards}
Given that cybersecurity stems from conflict between attackers and defenders targeting one or more vulnerabilities,
creating a capturable {\em many-to-many relationship} is essential when introducing cybersecurity concepts. Thus, the
cybersecurity cards should represent this relationship, where multiple attacks can target multiple vulnerabilities that
can, in turn, be mitigated or countered by multiple defences. While CyBOK does contain information about these
relationships, it is hard to infer these from implicit references within the reference material.
% how do we derive the cybok implicit relationships and link this to the example in next paragraph
In Figure~\ref{fig:carddesign}, we can see that the vulnerability card {\em "Blind Trust of User Input"} is linked to a
set of identifier codes \circled{3} for a number of related attacks and defences. This example shows a link to the
{\em "Command Injection"} and {\em "Memory Thief"} attacks. The first attack involves the execution of unauthorised
commands to a system (which may be input by a user) and the second involves the stealing of confidential information
from memory. In contrast, two defence examples are shown as links to the attacks and the vulnerability, which include
{\em "Code Assertions"} and {\em "Input Sanitisation"} which involve monitoring code execution and sanitising user
input to eliminate malicious code or escape characters, respectively.

\subsection{Expected Usage}

We anticipate that the structuring and indexing employed by the design of the deck of
cards will provide opportunities for easy exploration of complex
cybersecurity topics. Thus, an individual with little-to-no experience in this
area could start with one known or familiar topic, typically a vulnerability, and
use the linkable relationships between cards to reach other topics. We believe this would allow
a more natural feel for progression and may appear less daunting compared
to trawling through an encyclopedic knowledge base such as CyBOK. The use of a playing cards
format is one that is interactive and can facilitate communication between
participants in exploration exercises and allows one to claim ownership of
what is being communicated by holding the card representing a piece of cybersecurity
knowledge. Using General cards as a starting point to understand core
information, and then progressing on to more concrete attack-defence scenarios, might
provide a more gentle learning pathway for novice users.

==> sections/cards_2.tex <==
%-------------------------------------------------------------------------------
\section{Cybersecurity Cards -- Version 2}
\label{sec:cards1}
%-------------------------------------------------------------------------------

Upon review of the results from the evaluation questionnaire, the
cybersecurity cards were in places redesigned and the new deck is hereafter
referred to as {\em Version 2}. As well as providing the subset of the Version 1 cards for viewing, the equivalent
subset for Version 2 of the cards have also been made available and can be found
online\footnote{\url{https://anonymous.4open.science/r/cybersecurity_cards-9F00/} (anonymous repository for double-blind reviewing purposes)}. The full set of cards will be made publicly available under the CC BY-NC-SA Creative Commons license after the research project ends in January 2024.

% \MMcomment{Potentially have a table to showcase the key comparison points / differences between v1.0 and v1.1}

\subsection{Structural Redesign}

One of the limitations that required addressing was with regard to
the number of cards in the deck, which some participants felt was
too high and {\em "difficult to handle and understand (PM7)"}. As described
in Section~\ref{sec:cards}, Version 1 of the deck has 109 cards in total,
consisting of 32 attack cards, 30 vulnerability cards and 47 defence cards,
categorised under one of the 15 General cards. In contrast with a standard
deck of playing cards used for the likes of Solitaire and Poker, which has 52 cards,
Version 1 of our cards has more than double this amount resulting in it being
perceived by participants as hard to handle. Therefore, reducing the number of cards in
Version 2 of the cards to a more familiar number will likely be better received, whilst
still retaining the goals from Version 1 of providing introductory knowledge of cybersecurity,
facilitating independent learning and self-efficacy, and providing an interface for
discussion of key topics.

In Version 2, the first major revision is reducing the number
of cards in the deck. The first decision made with regard to this was the removal of General
cards, given that participants specified the least used cards to be the General
cards which denote a {\em type} of attack, defence or vulnerability card. One participant
stated that {\em "general cards gave some idea about the content (PF6)"}, however this does
not justify their need to be placed within the deck. Instead, Version 2 of the cards come
with a {\em glossary} document which provides a description of each of
the General cards, alongside a symbol associated with the type in the top left of the card
to help improve readability and visibility. This reduces the number of cards in Version 2
to a total of 70 cards, made up of 20 attack, 20 vulnerability and 30 defence cards. On each
of the attack, vulnerability and defence cards, the symbol for its associated type found in the
glossary is in the top left corner (Figure~\ref{fig:manytomanycardsv2}).
By providing a glossary, users can refer to this sheet as a form of
guidance when looking at devising particular cybersecurity scenarios, as
well as addressing the lack of usage of general cards and poor handling due to
having a large deck. The descriptions of each of the types of attack, defence or vulnerability
in the glossary improve on the grammar and readability from those present in the General cards in
Version 1. Furthermore, while the symbol icons stay the same, we also propose two new classes of vulnerability.
First, {\em Human} is split into {\em User} and {\em Management} which captures the impact of
vulnerabilities from careless or malicious user insiders, but also bad understandings from management in
organisations. Second, we provide a {\em System} vulnerability type which relates to computer infrastructure,
to better capture attacks and defences that target the computer system, as opposed to assuming that this is
simply a result of badly written code or poorly configured execution environments as observed in Version 1.
The glossary can be found in Appendix~\ref{app:glossary}.

In terms of general design, examples of Version 2 cards can be seen in
Figure~\ref{fig:manytomanycardsv2}. The red background is made
slightly lighter making it easier on the eyes, with the symbols
watermarked in the background of the card also made lighter to
maintain focus on the content of the card whilst also still
highlighting the card type. Further, the fonts across the cards
were changed to improve clarity. Finally, defence cards are now
more akin to a stop sign which helps distinguish them with the
attack cards.


\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{img/relationshipv2.pdf}
    \caption{\centering Example of a Many-to-Many Relationship Within Version 2}
    \label{fig:manytomanycardsv2}
\end{figure}

\subsection{Relationship Clarification}

The next revision made in Version 2 of the cards is a clarification
of the links between the cards to highlight relationships between
various vulnerabilities, attacks and defences, which was described to be inadequate. As shown in
Figure~\ref{fig:manytomanycardsv2}, the card identifiers which were
initially positioned in the top right corner (Figure~\ref{fig:carddesign})
are now replaced with a symbol and a card number related to each type
which is positioned in the top left corner \circled{1}. As previously mentioned,
this symbol corresponds to its associated type which is defined in the glossary
(Appendix~\ref{app:glossary}). The card number is the number of the card within a type.
For example, {\em Command / Data Injection} is card number 2 for the {\em Injection}
attack type.

As well as this, instead of related attacks and defence codes listed at the bottom of
the vulnerability cards, attack and defence cards explicitly showcase related
vulnerability cards denoted by the relevant type symbol(s) made darker along with
the card number(s) for the type of vulnerability. Similarly, vulnerability cards
use the same format for showcasing the related attacks and defences
\circled{2}+\circled{3}. The defence cards do not explicitly refer to
specific attacks for which they target as, given the dynamic nature of
cybersecurity and evolving threat landscapes, a single defence strategy
could be employed to defend against multiple attacks or mitigate the chance
for vulnerabilities to be exploited. Instead, links are given to vulnerabilities
but the aim behind this is to encourage card users to intuitively tackle
attack vs. defence strategies by learning from the content within the cards and
explicitly highlight the relationships to various attacks and defences.


\subsection{Evaluation of Version 2}

To evaluate the second version of the cards, we make use of the same workshop format described in
Section~\ref{sec:evaluation}. However, the difference here pertains to the demographic of the participants. In this
second workshop, we recruited 23 participants with ages ranging from 10 to 15 years old (mean 12.8 years), of which
7 were female and 16 were male, from either primary or secondary school. When asked to describe any experience and/or
skills they may already have with cybersecurity, one participant stated they know the basics, one saying that
passwords are important, one stating they know about hacking, and all other participants saying they have either no
experience (17) or are unsure (3). When asked about experience or skills with coding, two participants stated they had
limited experience with Python programming, six stating they have used Scratch or other block-based visual programming
tools, with the remainder (15) having no programming experience. Furthermore, only 2 participants stated they had
experience with secure coding, with one neutral and the remainder either disagreeing or strongly disagreeing with this.
After the workshop, the participants were given the same questionnaire to answer as those received in the first workshop
(Appendix~\ref{app:questionnaire}). For subsequent discussion, we will discuss the results of the evaluation on the
second version of the cards on the same themes as the first version presented in Section~\ref{sec:results1}: (1)
{\em providing a knowledge base, including: cybersecurity concepts, scope and relationships
(vulnerability-attack-defence)}; (2) {\em independent learning and self-efficacy}; (3) {\em providing an interface for
discussion on key cybersecurity topics}; and (4) any {\em drawbacks of using the cards}.

\subsubsection{Providing a Knowledge Base}
\label{sec:provideknowledge2}

For the first theme of determining whether the cards provided introductory cybersecurity knowledge that supports
learning in a well-documented manner, we look at the four items (\textbf{a--d}) in Question 1 of the questionnaire in
Appendix~\ref{app:questionnaire}. For individual concepts \textbf{(a)}, 17 of the participants agreed that the cards
provided them with knowledge of cybersecurity concepts, terminology and topics (6 somewhat agree, 4 agree and 7 strongly
agree) with 3 participants scoring neutral and 3 somewhat disagreeing with this. For wider scope \textbf{(b)}, 17
participants agreed (3 somewhat agree, 6 agree and 8 strongly agree) that the cards provided them with this knowledge,
with 2 disagreeing and 4 remaining neutral. For relationships between attacks, defences and vulnerabilities \textbf{(c)},
16 agreed (6 somewhat agree, 3 agree and 7 strongly agree) that the cards facilitated the understanding of the links
between cards that capture the vulnerability-attack-defence dichotomy that is present in cybersecurity, with 4 neutral
and 3 disagreeing. Finally, with regarding to cybersecurity terminology \textbf{(d)}, 14 participants agreed (4 somewhat
agree, 4 agree and 6 strongly agree) that the cards provided them with knowledge on terminology. Three participants
disagreed with this and the remaining 6 were neutral.

%% questions 1(a-d)
%% 1a -- 3 somehwat disagree, 3 neutral, 6 somewhat agree, 4 agree, 7 strongly agree
%% 1b -- 2 disagree, 4 neutral, 3 somewhat agree, 6 agree, 8 strongly agree
%% 1c -- 3 disagree, 4 neutral, 6 somewhat agree, 3 agree, 7 strongly agree
%% 1d -- 3 disagree, 6 neutral, 4 somewhat agree, 4 agree, 6 strongly agree


\subsubsection{Independent Learning and Self-Efficacy}
\label{sec:independentlearning2}

The theme of independent learning and self-efficacy relate to items (\textbf{e,f}) in Question 1. The first item
asked participants if the cards helped them undertake independent learning of cybersecurity \textbf{(e)}. We found that
for the second version of the cards, 11 participants agreed (2 somewhat agree, 4 agree, 5 strongly agree), 7 were
neutral and 5 disagreeing (1 strongly disagreeing). For the second item, we asked if the cards provided access to
cybersecurity knowledge without the presence of an expert. We found that 13 participants agreed (3 somewhat agree, 3
agree and 7 strongly agree), with 5 participants neutral to this and 5 disagreeing (1 strongly disagreeing).

%% questions 1(e-f)
%% 1e -- 1 strongly disagree, 4 disagree, 7 neutral, 2 somewhat agree, 4 agree, 5 strongly agree
%% 1f -- 1 strongly disagree, 4 disagree, 5 neutral, 3 somewhat agree, 3 agree, 7 strongly agree


\subsubsection{Providing an Interface for Discussion}
\label{sec:provideinterface2}

The final theme explored relates to the cards providing an interface for discussing key cybersecurity topics and relates
to items (\textbf{g, h}) in Question 1. The first question related to this theme asked participants if the cards enabled
them to discuss cybersecurity topics with an expert \textbf{g}. We found that 14 participants agreed with this (3
somewhat agree, 5 agree and 6 strongly agree), with 6 participants remaining neutral to this and 3 disagreeing (1
strongly disagreeing). The final question in this theme asked them if the cards enabled them to hold discussions on key
cybersecurity topics with others in their group \textbf{h}. We found that 14 participants agree with this (4 somewhat
agree, 4 agree and 6 strongly agree), with 5 participants neutral and 4 disagreeing with this.

%% questions 1(g-h)
%% 1g -- 1 strongly disagree, 2 disagree, 6 neutral, 3 somewhat agree, 5 agree, 6 strongly agree
%% 1h -- 4 disagree, 5 neutral, 4 somewhat agree, 4 agree, 6 strongly agree


\subsubsection{Understanding Drawbacks of Version 2}
\label{sec:limitations2}

In a similar manner to Version 1 of the cards, the next three questions were designed to gather understanding on any
limitations of the cards and whether there may be any improvements that can be made. Given that the same investigation
was performed for Version 1, the aim here is to observe whether the design and structural changes we made using the
findings to revise Version 1 of the cards have allowed for better fulfilment of the goals of the research questions
described in Section~\ref{sec:cards}. In Question 2, we asked participants whether there were any categories or subset
of cards not used by them in the workshop. The difference in this question compared to the same questionnaire employed
for evaluating Version 1 is due to the removal of the General cards and that they are replaced with a Glossary. Thus, in
Appendix~\ref{app:questionnaire}, we refer to {\em Question 2 (Version 2 Evaluation)} which includes the Glossary as an
option, as well as cards within a specific category for each of the classes. We found that the least used item was the
Glossary (7 participants) and Race Condition (7), with the next least used cards being Injection (6) and Memory (6) attack
cards, Mitigation (6) and Education (6) defence cards, and System and Environment vulnerability cards. Looking at
Question 3 to understand why these types of cards (excluding the glossary) in particular were not used, some
participants mentioned that they ``didn't need them'' (PM8), were ``unnecessary'' (PM20) or ``don't know'' (PM9). One
reason for this may be due to cards such as race conditions sound more intimidating and/or complex, in particular for
those are less experienced (in this case participants from primary or secondary school, in comparison with students from
higher education backgrounds in Version 1). With regard to the glossary, some participants stated that ``nobody reads
the glossary'' (PF10), suggesting that this was not needed and the cards alone for some participants were enough to
facilitate learning and understanding of key cybersecurity topics. Interestingly, some participants had stated that
they had ``used all the cards'' (PM4, PF6), with some others giving a similar reason yet selecting many (if not all)
checkboxes for all cards. In Question 4, we asked participants if there were any other improvements to the cards they
would like to suggest. Most participants (14) said ``No'' to this question, however one participant suggested to use
``simple wording'', which may correlate with why certain cards (e.g. Race Condition or Memory attacks) were not used.
As well as this, three participants suggested to make the cards ``easier to use'' (PM2,PM14), however any suggestions as
to how they might think this could be achieved were not elaborated.

% Question 2 - which category/subset cards not used, tick all boxes
%% Note: This question is different as we no longer have general/detailed cards, we refer to
%%       "Question 2 (Version 2) of cards".
%%
% Glossary - 7
% Attack cards (in general) (fully red cards) - 4
% Vulnerability cards (in general) (cards with half red/half white diagonal) - 4
% Defence cards (in general) (white cards with red border) - 5
% Attack -- Injection cards - 6
% Attack -- Memory cards - 6
% Attack -- Race condition cards - 7
% Attack -- Side channel cards - 5
% Attack -- Authentication cards - 5
% Attack -- Web cards - 4
% Attack -- System cards - 5
% Attack -- Human factors cards - 4
% Defence -- Detection cards - 5
% Defence -- Mitigation cards - 6
% Defence -- Education cards - 6
% Defence -- Prevention cards - 4
% Vulnerability -- Code cards - 5
% Vulnerability -- System cards - 6
% Vulnerability -- Environment cards - 6
% Vulnerability -- User cards - 2
% Vulnerability -- Management cards - 4
% Other - "I used all of them", "other", "no"

%\subsubsection{Future Work}

==> sections/conclusion.tex <==
%-------------------------------------------------------------------------------
\section{Conclusion}
\label{sec:conclusion}
%-------------------------------------------------------------------------------

Cybersecurity is a complex subject area that is constantly changing due to the
dynamic nature of vulnerabilities, attacks and defences. Unfortunately, because
of this, many users of computer systems who may have little-to-no knowledge of
cybersecurity are left vulnerable. Many organisations provide basic cybersecurity
training and implement best-practices, but the question as to whether users truly
understand the impact of these measures and the consequences of not adhering to them
remains.

Existing knowledge bases such as CyBOK have the potential to provide key information,
but often fall into a trap of being a vast body of knowledge that is hard to traverse
and understand relationships between the key topics they aim to provide access to.
In this work, we propose an approach that makes use of a playing cards format for introducing
and interfacing with cybersecurity topics. The novel contributions of this work include
designing a deck of cybersecurity cards that act as a more accessible and digestible index
for learning key cybersecurity topics informed by the CyBOK knowledge base, facilitate
independent learning of key topics and promote understanding of the various relationships
found in the cybersecurity ecosystem, addressing the limitations of existing solutions/activities
that aim to facilitate learning. Upon evaluation, we found that the cybersecurity
cards did in fact provide an accessible knowledge base and facilitate independent
learning of key cybersecurity topics. Further, we also found that relationships between
vulnerabilities, attacks and defences were understood by participants. While most
responses promote the success of our approach, there were limitations with respect to
the design of the cards which impacted the learning of some participants. Addressing
these limitations, we then propose the next version of our card deck (Version 2)
focusing mainly on the design of the cards to improve physical handling, as well as
better highlighting the links between vulnerabilities, attacks and defences.

In conclusion, our proposed cybersecurity cards provide a comprehensive and effective tool that
allows for the learning of key cybersecurity topics which also promotes discussion. This design
not only allows for non-technical learners to gain introductory knowledge of
cybersecurity, but also promotes creative independent learning and allows users
of the cards to analyse and devise various cybersecurity scenarios and how vulnerabilities,
attacks and defences may play a role in them.

==> sections/discussion.tex <==
%-------------------------------------------------------------------------------
\section{Discussion}
\label{sec:discussion}
%-------------------------------------------------------------------------------

The aim of this research is to evaluate how the cybersecurity cards provided a clear communication of key
cybersecurity topics and an interface for discussing them, leveraging the information from the CyBOK knowledgebase. To
investigate this, we were guided by the research questions proposed in Section~\ref{sec:cards}. In this paper, we
provide an evaluation of two versions of the cybersecurity cards and subsequent discussion will encompass both sets of
results and follow each research question in turn.

\subsection*{\normalsize RQ1: Do the cybersecurity cards provide introductory cybersecurity knowledge to novice users?}

Cybersecurity is often overlooked as a subject due to issues such as perceived technical difficulty, steep learning
curves and a requirement of specialist knowledge and/or expertise. In industry, for example, the lack of cybersecurity
professionals has been linked to a lack of practical cybersecurity content within learning
materials~\cite{caldwell2013plugging}. While CyBOK aims to rectify this learning gap, traversing the knowledgebase and
understanding key concepts and topics in cybersecurity requires prior knowledge, as evidenced by the fact that the
primary usage of CyBOK involves curricula development for higher education programmes~\cite{hallett2018mirror}, and thus
may not be considered accessible for novice individuals. In this work, we show that our cybersecurity cards achieved a
positive result with regard to providing introductory knowledge of key cybersecurity topics to novice users. Specifically,
we found that most participants from the first workshop in higher education agreed (Section~\ref{sec:provideknowledge1})
with this, and our second workshop involving school children -- who described themselves as having much less
cybersecurity and secure coding experience/skills -- also agreeing with this (Section~\ref{sec:provideknowledge2}).

\subsection*{\normalsize RQ2: Do the cybersecurity cards provide material for expressing interpretation of key topics that supports independent learning and self-efficacy?}

One of the concerns surrounding cybersecurity relates to the preconception of steep learning curves and a requirement of
specialist knowledge and expertise~\cite{asen2019you,bahizad2020risks}, which is a problem that is not adequately
managed by the CyBOK knowledgebase. From our evaluation of the cards, we found that most of our participants in higher
education from the first workshop agreed they were able to understand key cybersecurity topics independently (Section~\ref{sec:independentlearning1}).
Interestingly, we found that half of the primary and secondary participants in the second workshop agreed with this (Section~\ref{sec:independentlearning2}),
with the remainder equally neutral or disagreeing. It appears that removing the general cards and replacing them with a
glossary may have impacted this may have impacted this, backed up by statements from the participants saying that nobody
reads the glossary. Thus, an important consideration is how this information could be better presented. In terms of
self-efficacy, we found that the higher education participants agreed that even without a cybersecurity expert present
in the group, they were able to access cybersecurity knowledge solely using our cybersecurity cards. For the primary and
secondary school participants, more participants agreed on this compared to understanding topics independently.

\subsection*{\normalsize RQ3: Do the cards act as an index for the CyBOK knowledgebase, which provides an interface for discussion on key cybersecurity topics?}

Given that the primary use cases of the CyBOK knowledgebase relate to the construction of educative teaching
material and the fact this requires existing specialist knowledge on topics within the CyBOK KAs to be
developed on further~\cite{hallett2018mirror}, it is clear that it is not easy to traverse the CyBOK
knowledgebase. Other cybersecurity learning solutions which make use of
a playing card format~\cite{denning2013control,thomas2019educational,anvik2019program} also show some success
in this aspect, for example arguing that a gamified cards approach can help provide a reachable foundation for
providing digestible cybersecurity information. In this work, while we also make use of a playing cards format, the
intended use is not in the context of games which have shown to have limitations with regard to perceptions of quality
and effort related to learning game mechanics. In any case, many of these existing approaches are either designed for
those with existing cybersecurity knowledge~\cite{swann2021open,trickel2017shell,cybokctf} or do not make use of a
peer-reviewed and well-established knowledge foundation such as CyBOK~\cite{denning2013control,anvik2019program}. It has
been shown that the value of security information and how well it is understood or perceived as actionable depends
strongly on the source~\cite{redmiles2020comprehensive,rader2015identifying}. The first version of our cybersecurity
cards show that the majority of participants agreed they were able to discuss key topics with cybersecurity experts that
periodically checked in on them, as well as with other members in their group (Section~\ref{sec:provideinterface1}).
For the second version of the cards, we found that most participants also agreed, with more strongly agreeing compared
to those in further education using the previous cards. While some participants in both cases disagree with this (1
strongly disagreeing in both workshops), this may be due to reasons such as simply not wanting to discuss topics with
the experts. Interestingly, in the second workshop, we found that more participants disagreed that the cards enabled
them to hold discussions with others in their group. This could be due to a lack of interest in doing so, or potentially
they simply did not know they could do that. Ultimately, CyBOK has been shown to lack depth, particularly in the aspect
of practical experience such as discussing key topics, which is essential for mastering cybersecurity
skills~\cite{manson2014case,hallett2018mirror}. From our evaluation, we found that our cards can provide this to even
novice users of different age groups.

\subsection*{\normalsize RQ4: Do the cards provide links between key cybersecurity topics, allowing for the capture of various scenarios?}

In the evaluation questionnaire, we asked participants whether the cards provided them with knowledge about
the relationships between attacks, defences and vulnerabilities (Section~\ref{sec:provideknowledge1}). We
found that the majority of participants agreed with this. This is further strengthened given that most
participants in the first workshop also agreed the cards promoted discussion of key cybersecurity topics with both
experts and other members in their groups (Section~\ref{sec:provideinterface1}), with similar results seen in the
second workshop with primary and secondary school participants (Section~\ref{sec:provideinterface2}). While the
CyBOK knowledge base does encapsulate the attack-defence-vulnerability dichotomy, it is difficult to identify
whether some topics focus on a single predominant theme or whether it spans across various
themes~\cite{gonzalez2022exploring}. Furthermore, it has been shown that because of this difficulty, these links could
be identified from series of keywords which are only meaningfully extracted via specialised algorithms such as topic
model analysis~\cite{gonzalez2022exploring,hallett2018mirror}. With regard to other learning approaches for
cybersecurity, Capture The Flag (CTF) activities manage to highlight links between attacks, defences and 
vulnerabilities as well by prioritising the focus of finding vulnerabilities which can help users understand
how they present themselves, how they can be targeted and how to protect against attacks which target
them~\cite{trickel2017shell,swann2021open}. Interestingly, some CTFs have been designed leveraging CyBOK as
its foundational information source or inspiration~\cite{cybokctf}. However, the disadvantage to these
approaches is that CTF competitions rely on technical expertise of computer systems, with activities
involving the use of command-line tools or requiring, at a minimum, a basic understanding of cybersecurity
concepts in order to progress in finding vulnerabilities~\cite{mcdaniel2016capture}. We show that our
cybersecurity cards provide the introductory cybersecurity knowledge for novice users, whilst also allowing
them to devise various cybersecurity scenarios that encapsulate the vulnerability-attack-defence dichotomy.

% TODO:!!
\subsection{Reported Limitations and Future Work}

From the evaluation of the first version of the cards, we identified some limitations from participant responses. First,
some participants felt the overall number of cards was too high and some cards (e.g. General cards) were not really used.
In the second version, this prompted a minimisation of the deck to improve physical handling, whilst also adhering to
the primary goals, and the replacement of General cards by a glossary that can be referred to whenever needed. In the
second workshop using the updated cards which replaces the General cards with a glossary, we found that there were no
suggestions regarding the number of cards causing any difficulties related to usage. However, some participants felt the
glossary was not useful and in some cases was not used at all. Because of this, a point of future work would look into
how such information could be portrayed differently. One potential solution to this could be to make use of additional
introductory cards (Figure~\ref{fig:introcard}), which may help provide this information in a different way using the
deck of cards already being interacted with, compared to how the glossary was perceived.

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{img/introcard.png}
    \caption{\centering Introductory Card Example}
    \label{fig:introcard}
\end{figure}

Second, the layout and written content of first version of the cards were described as difficult to go through by
participants in the first workshop. For the second version of the cards, we improved the contrast of the red colour,
as well as the layout of card elements (e.g. positioning of symbols) to help improve clarity. In the second workshop,
none of the participants explicitly suggested any design changes to the cards. However, the number of participants who
agreed that the cards provided knowledge on the relationships between attacks, defences and vulnerabilities could be
improved. One potential design change that may improve this result is to better visibly distinguish between the
different classes of cards. In previous work, it has been studied whether different colours of warnings can affect one's
perception of risk~\cite{young1991increasing,leonard1999does}. For example, the same red color could be used for attack cards as it is typically associated with
danger and a higher perceived relative amount of risk. An orange or amber colour is typically used for warnings and
the colour yellow for caution, which could be used to signal the vulnerability cards as they


Second, the layout of the cards and written content were identified as
difficult to go through, and the colour-coding was also suggested to be updated. A new version should think about
colour contrast and the layout of various card elements (such as positioning of symbols) to improve clarity. Finally,
the links between the cards should also be revised in a new version of the cards, given that some participants stated
they only focused on attacks and defences. One of the limitations of other playing cards
approaches~\cite{denning2013control,anvik2019program} was that attacks are typically highlighted first, which
does not help users understand how attacks present themselves via vulnerabilities and how to protect against
them (defences). While this could be due to participants with limited knowledge thinking in terms of attacks vs.
defences and neglecting related vulnerabilities, it may also be that they find it hard to make links between
attacks and defences from the use of codes within the vulnerability card. This issue of readability to form
these links from vulnerabilities may be preventing them from making use of other vulnerability cards as a starting
point. In either case, the focus of centering on vulnerabilities is an important point, and a clear and concise
design that focuses on improving this will likely play a pivotal role in improving not only independent learning
and self-efficacy, but also enable the devising of various cybersecurity scenarios.

==> sections/evaluation.tex <==
%-------------------------------------------------------------------------------
\section{Evaluation}
\label{sec:evaluation}
%-------------------------------------------------------------------------------

The logical next step after designing the cybersecurity cards was to conduct a user
evaluation to see if the participants could use the cards, and whether the cards
provided a clear communication of these topics and an interface for discussing them.

\subsection{Methodology}

% The focus of the evaluation of the cybersecurity cards was to determine the extent to
% which the knowledge and understanding the cards provided the participant with key
% information and learning regarding cybersecurity topics.
Participants were recruited to take part in a workshop, advertised to university students, where they interacted with
the cybersecurity cards in order to analyse and devise a cybersecurity scenario. Ethical approval was granted by the
University ethics committee for the workshop recruitment and procedure before the study took place. A participant
information sheet was provided via a link in the online registration form, as well as being used to obtain written
consent from participants. Furthermore, the workshop was held in Spring 2022 and we had a special clause added to state
we would follow local government guidelines on the Covid-19 protocol~\cite{covidspring22} which provided guidance on
reducing risks from transmitting Covid-19, such as staying home if participants had symptoms or tested positive for
Covid-19. In total, we managed to recruit 13 participants but only 11 had usable data. Upon registration for the
workshop, we found that the 11 participants were masters-level students (8M, 3F) who were between 22 and 35 years old
(mean 26.3 years). The participants were enrolled in a conversion masters program in computer science and came from
either an engineering (6), mathematics (3), computing (1) or biology (1) background. When asked if the participants had
any prior experience or skills with cybersecurity, only one participant mentioned they had experienced anomaly detection
but others stated they had no prior experience or skills in cybersecurity. Further, when asked if they had any
experience or skills with secure coding, 8 of the participants said they had no experience or skills with secure coding,
2 responded neutral and 1 said they had some experience. We hypothesise that the low number of participants to be
attributed to the Covid-19 global pandemic leaving individuals with more dynamic priorities and commitments.

Before the workshop took place, the participants were split into three groups (consisting of three or four participants).
During the workshop, participants were first given a presentation to introduce the cybersecurity deck of cards. Each
group was then given a deck of cards each where they could browse through and create links between cards themselves,
devising various cybersecurity scenarios. Cybersecurity experts were also present in the room, being available whenever
participants may have had questions or wanted to hold a discussion, and only periodically went round the groups to
check on them if nothing was asked. After the workshop, each participant was individually asked to fill in a
self-assessment questionnaire online (Appendix~\ref{app:questionnaire}) on how using the cards contributed to the
following themes: {\em providing a knowledge base, including: cybersecurity concepts, scope and relationships
(vulnerability-attack-defence)}; {\em independent learning and self-efficacy}; and {\em providing an interface for
discussion on key cybersecurity topics}. The rationale behind this questionnaire was to collect both quantitative and
qualitative data regarding a participant's experience of interacting with the cybersecurity cards. The quantitative
aspect of the questionnaire (Q1) makes use of a 7-point Likert scale, ranging from strongly disagree to strongly agree,
to assess the performance and effort from participants while using the cards. The qualitative aspect (Q2--5) aims to
understand motivations and thoughts behind using the cards. Question 2 and 4 gave participants a series of options
(checkboxes), which were then coupled with a follow-up question (Q3 and Q5 respectively) to further elaborate on their
choices. Two experienced postdoctoral researchers independently analysed and coded the qualitative responses, grouping
them into themes, which were then discussed systematically and final agreements on codes were made in consensus.
This analytical technique has been applied successfully in various bodies of
work~\cite{zade2018conceptualizing,chinh2019ways}. The data from questionnaires is presented as italics in quotation
marks, alongside a participant ID (e.g. PF6 or PM11 for a female or male participant respectively) where relevant. As
well as this, mappings to the aforementioned themes were also decided in consensus among the coders.

\subsection{Results}
\label{sec:results1}

For subsequent discussion, the results from the questionnaires will initially follow
three themes: (1) {\em providing a knowledge base, including: cybersecurity concepts,
scope and relationships (vulnerability-attack-defence)}; (2) {\em independent learning and
self-efficacy}; (3) {\em providing an interface for discussion on key cybersecurity topics};
and (4) any {\em drawbacks of using the cards}.

\subsubsection{Providing a Knowledge Base}
\label{sec:provideknowledge1}

For the first theme the aim was to determine whether the cards provided participants
with introductory cybersecurity knowledge that supports learning in a well-documented
manner, we look at the first four items (\textbf{a--d}) in Question 1 of the
questionnaire (Appendix~\ref{app:questionnaire}). On average, 80\% of the participants agreed
that the cybersecurity cards provided them with knowledge of cybersecurity concepts,
terminology and topics. For individual concepts \textbf{(a)}, 10 participants
{\em agreed} that the cards provided them with knowledge of individual
cybersecurity concepts, with three of them strongly agreeing. One participant had a
neutral response. For knowledge about wider scope \textbf{(b)}, 9 participants
{\em agreed} that the cards provided them with this knowledge, with four of
them strongly agreeing. For the third item regarding knowledge about the relationships
between attacks, defences and vulnerabilities \textbf{(c)}, 10 participants
agreed the cards provided this knowledge with three strongly agreeing. Finally, for the
fourth item regarding cybersecurity terminology \textbf{(d)}, only 7 agreed
the cards provided the participants with knowledge on terminology. Two of
the participants scored neutral and two responded with somewhat disagree.
% As a whole, it is
% clear that
% the cards have indeed achieved a positive result with regard to %with 9 of the participants declaring that
% % the cards have provided
% providing participants with knowledge of fundamental cybersecurity concepts.
% Interestingly, the lower scoring for cards providing participants with cybersecurity terminology
% may be due to the text on the cards using too much technical terminology.


\subsubsection{Independent Learning and Self-Efficacy}
\label{sec:independentlearning1}

The theme of independent learning and self-efficacy relates to items \textbf{(e,f)}
(see Appendix~\ref{app:questionnaire}). The first question \textbf{(e)} asked participants if
the cards enabled them to undertake independent learning about cybersecurity. We found that 8 of
the participants had
agreed with this statement with three strongly agreeing. One participant disagreed
with this, while the other two were neutral. The second question \textbf{(f)} asked
participants whether the cards provided access to cybersecurity knowledge when one of the
rotating cybersecurity experts was not present in the group. We found that 9 out of the 11 participants agreed with this, with 1 participant stating they were neutral and another
disagreeing with this statement.


\subsubsection{Providing an Interface for Discussion}
\label{sec:provideinterface1}

The theme of providing an interface for discussion relates to items \textbf{(g,h)} in
Question 1 of the questionnaire (see Appendix~\ref{app:questionnaire}). 
The first question relating to this theme, \textbf{(g)}, asked participants if the cards
enabled them to discuss cybersecurity topics with the expert. We found that 9 participants
said they agree, with 3 participants strongly agreeing that the cards enabled them to discuss
topics with the expert in their group. One participant strongly disagreed with this.
% This could
% be due to reasons such as already having knowledge of cybersecurity topics being discussed
% at the time or simply not wanting to discuss topics with the experts.
The second question in
this theme, \textbf{(h)}, was used to determine whether the cards allowed participants to hold
discussions on key cybersecurity topics with others in their group, without the cybersecurity
expert. Interestingly, 7 of the participants agreed that the cards enabled a discussion with
others. Three participants were neutral to this and only one participant said they disagreed
with this statement.
% While overall we see a positive outcome regarding the cards providing an
% interface for the discussion of key cybersecurity topics, it is important to determine what was not
% clear and why this was the case, as well as understanding how the cards could be improved.


% \subsubsection{Understanding Limitations}
\subsubsection{Understanding Drawbacks Of Using The Cards}
\label{sec:limitations1}

The next three questions in the evaluation questionnaire were designed to help
uncover and understand any limitations of the first deck of cards, such that
improvements can be made to better fulfill the goals of the research questions described in
Section~\ref{sec:cards}. The first step was to determine which category or subset of
the cybersecurity cards the participants did not use and why this was the case.
Overall, the category or subset of the cards that were used the least were the general
and detailed defence and vulnerability cards. Looking at their responses in Question 3
regarding why these were the choices, one participant stated that {\em "general cards
gave some idea about the content" (PF6)} with another mentioning that they were only
{\em "engaged in attack and defence"} (PM11). With this said, however, most participants
described that they had used all of the categories, for example stating they had used
{\em "at least one card [from] each"} (PM1) or only to {\em "concentrate on a few cards"} (PF9).
This provokes the notion that some participants made some selections in Question 2 under the
presumption that these cards were not used for primary interactions but not necessarily that
they were not looked at or thought about.

For Question 4, we asked participants about how they may think the cybersecurity cards
could be improved based on a few checkboxes that they felt applied to their
experience. 5 of participants recorded that the number of cards was too high. This
may be due to the use of a physical medium and the number of categories and types of
each General card. This corresponds with 3 of the participants recording that there
were too many types or categories. As well as this, 5 of the participants also
recorded that both the color coding of types/categories were not clear, as well as the
relationship between the cards. In Question 5, one participant stated that {\em "Threat cards
[were] difficult to handle/understand"} (PM7). This may also correspond with
the feeling that the number of cards was too high, but also that perhaps the difficulty
of understanding the cards may be linked with the relationships between them, as well as
the terminology used. In contrast to this, however, one participant mentioned that the {\em "Cards
provides an entry point for more detailed scenarios of cyber security and helps to create
relationship between attack and defense situations more clear"} (PM4). Interestingly, 3 participants
recorded that the information on the cards were too abstract, with no participants stating that
they were too detailed. Thus, this helps reinforce the understanding that the difficulty relating
to understanding the cards may be linked to a lack of clarity on the relationships between them.
Further, one participant suggested an {\em "update [to] the colour-coding of the cards"} (PM4),
as the red color with minor style changes leaves them {\em "difficult to go through"}.
% TODO: Are we going to talk about the digital medium stuff?
% Finally, 4 participants stated that they would prefer to have the combination of both
% physical and digital cards - 1 person said just prefer to have digital cards..

% \MMcomment{Add a small paragraph here explicitly stating the key takeaways from limitations of v1.0 (i.e. what is needing to be changed in v1.1)}

% 5 - \#cards too high
% 0 - \#cards too low
% 3 - too many types/categories
% 2 - logos and icons not clear
% 5 - color coding of types/categories not clear
% 5 - relationships between cards not clear
% 3 - information on cards too abstract
% 0 - information on cards too detailed
% 2 - information on cards too technical or difficult to understand
% 0 - prefer to have physical cards
% 1 - prefer to have digital cards
% 4 - prefer to have the combination of physical and digital cards

==> sections/introduction.tex <==
%-------------------------------------------------------------------------------
\section{Introduction}
\label{sec:introduction}
%-------------------------------------------------------------------------------

% In the information age, reliance on computer-based systems is constantly increasing.
Cybersecurity remains a fundamental concern to users of computer
systems, with security often being overlooked due to its portrayal as a subject
pertaining to issues of perceived technical difficulty, steep learning curves and a requirement of specialist
knowledge and/or
expertise~\cite{harknett2009cybersecurity,hoffman2011thinking,asen2019you}. While the security foundations of
computer-based systems have improved over time, limiting the potential for, or mitigating the effects of, attacks
arising from  vulnerabilities, requires the involvement of all users of these systems (e.g. the general
population) and is a necessary step to improve the understanding of cybersecurity~\cite{adams1999users}. Furthermore,
the increasing complexity and diversity of the threat landscape for
cybersecurity~\cite{wall2017crime,kaloudi2020ai,bahizad2020risks} further substantiates the need for improving
understanding of cybersecurity.

In the domain of software engineering, practical solutions to achieve this include activities such as the documentation
of vulnerabilities  of computer systems and updating respective knowledge bases. Open databases such as the Common
Vulnerabilities and Exposures (CVE)~\cite{cve} and Common Weakness Enumeration (CWE)~\cite{martin2011cwe}, have played
a pivotal role in raising the awareness of known vulnerabilities such that appropriate defensive measures can be
developed or updated. While these reference databases are well maintained, they may still appear
complex to the general population and may contribute to the already existing problems of inaccessibility and
specialist requirements that are pinned against the topic of cybersecurity. Because of this, several knowledgebases
have been developed to inform and underpin cybersecurity education and
training~\cite{martinintroduction,newhouse2017national,ncscmsc}, which aim to address these issues at a high-school or
higher-education level. Although they may be a useful learning resource for providing key cybersecurity knowledge, their
primary purpose is to be used by those who are already knowledgeable in cybersecurity to develop further curricula to
teach those who may have little-to-no knowledge of cybersecurity. Furthermore, among these knowledgebases, there may be
some key topics which are not covered, or the format and density of the knowledgebase may not be perceived as accessible
to novice users, both of which directly impacting one's ability to understand key cybersecurity topics but also make
links between these topics to capture real-world cybersecurity scenarios.

In this paper, we aim to address these limitations by proposing the use of a playing cards format as a medium to
provide: introductory knowledge of key cybersecurity topics, acting as an index for the CyBOK
knowledgebase~\cite{cybokwebsite,martinintroduction}; support independent learning and self-efficacy; and allow for
links to be made between key cybersecurity topics to capture real-world scenarios. The novelty of this work is three-fold.
First, we present the design principles for the cybersecurity cards to meet these provisions and develop an initial deck
of cards. Second, we provide an evaluation of these cards, carried out using workshop activity to devise cybersecurity
scenarios using participants at the level of education which existing knowledgebases target. The output of this evaluation
is a second revised deck of the cybersecurity cards. Third, we carried out the same workshop but with a different
demographic to the first, with participants at a primary and secondary school level, to not only compare and contrast
the findings from the first workshop but to also propose a third and final deck of cybersecurity cards.
%We first present the design principles
%for the cybersecurity cards to adequately meet these provisions and develop an initial deck of cards. The cards were
%then evaluated in a workshop where participants would interact with the cards to devise various cybersecurity scenarios.
%Observing the results and gathering insights from this workshop, we next provide a second version of these cards
%
%In this paper, we aim to facilitate access to and the communication of cybersecurity topics,
%to alleviate existing concerns and address the aforementioned requirements. Specifically,
%we propose the use of playing cards as a medium to represent key
%cybersecurity knowledge points. The advantages of using a playing cards format include:
%{\em accessible handling} in a physical medium~\cite{altice2014playing} and providing {\em digestible}
%information via a {\em tangible index}~\cite{malone2008use,setiaji2021development,arnab2015mapping} for
%cybersecurity knowledge bases.
%Each card proposed is designed to be self-contained, but allows for links to be made
%with other cards to build various cybersecurity scenarios surrounding the relationships
%between vulnerabilities, attacks and defences. We first present the design principles
%for the cybersecurity cards based on these requirements and developed an initial deck of these cards. The cards were evaluated in a workshop
%where interacting participants were split into small groups and supported by cybersecurity expert to help with
%using the cards whenever required. During the workshop, the cybersecurity experts were available at all times and would periodically check in
%on participants to make sure they understood what they were meant to be doing.
%% such that each group could hold discussions with varying perspectives provided by each expert.
%Overall, we found that the majority of participants in the workshop agreed that the
%cards provided them with knowledge of key cybersecurity topics and wider scope of these topics.
%As well as this, they also noted the cards provoked and promoted independent learning and
%self-efficacy, whilst also providing them access to key topics and making links between
%vulnerabilities, attacks and defences.
%Although the results were promising and demonstrate
%the success of our playing cards approach, there were some limitations reported by participants,
%including: the number of cards being too large and hard to handle; lack of use for certain
%types of cards; and the links between vulnerabilities, attacks and defences being unclear
%in some areas. Finally, to address these limitations, we propose several updates to the design of the
%cards and present the revised Version 2.

The remainder of this paper is organised as follows. Section~\ref{sec:background}
provides background and related work, as well as the selection
procedure we applied to the production of our cybersecurity cards using the CyBOK knowledge base and the
limitations of other approaches. The design principles
applied to the cybersecurity cards, as well as the initial implementation (Version 1), are described
in Section~\ref{sec:cards}. An evaluation of Version 1 of the cards and discussion of the results is provided in
Section~\ref{sec:evaluation} along with Version 2 of the cards. In Section~\ref{sec:cards1}, the evaluation and
discussion of the results from the second workshop using Version 2 of the cards is provided, ending with the design
of Version 3 of the cards. Finally, the paper concludes in Section~\ref{sec:conclusion}.

==> sections/related_work.tex <==
%-------------------------------------------------------------------------------
\section{Related Work}
\label{sec:related}
%-------------------------------------------------------------------------------

It has been shown that those in cybersecurity careers require a set of skills, involving
the abilities to carry out various tasks at any time in non-traditional environments and
adapt to the dynamic nature of these environments~\cite{niccs2015}.
Everyday users of any computer system gather information from
a wide array of sources, ranging from peer networks to (reputable) websites and television.
However, the amount of information that flows in a highly connected environment is
guaranteed to have a proportion of disinformation and the value of security information
depends strongly on its source~\cite{rader2015identifying}. Furthermore, strong information
is only useful so long as it is well understood and perceived as actionable~\cite{redmiles2020comprehensive}.
One factor that impacts how well security information is understood relates to having a correct
mindset that can adapt to a variety of highly dynamic and complex scenarios~\cite{thomas2019educational}.
Unfortunately, for novice individuals, cybersecurity may appear intimidating or confusing and
may require more specialist knowledge or guidance to promote adequate learning.

% Talk about CyBOK and other knowledge bases. Refer to hallett's paper to promote CyBOK.
To address this, various curriculum guidelines and knowledge frameworks have been developed for
cybersecurity, covering a range of fundamental topics ranging from software, hardware, networks and
cyber-physical systems. The Joint Task Force (JTF) on Cybersecurity Education propose a draft of
curricular guidance on cybersecurity to support educational efforts~\cite{bishop2017cybersecurity}.
They design a framework model for a body of knowledge that covers six knowledge areas which
several concepts span over, targeting specific disciplines and application areas which pertain to
the demographic of cybersecurity professionals. The National Initiative for Cybersecurity Education
(NICE)~\cite{newhouse2017national} is a cybersecurity workforce framework which aims to provide
a foundation for describing and sharing information about knowledge, skills and abilities in
cybersecurity to strengthen an organisation's cybersecurity. The NCSC propose a Certified Master's
Program that defines several pathways to address knowledge and skill gaps in cybersecurity education,
which describe what topics must be covered and to what depth~\cite{ncscmsc}. While all these frameworks
tend to agree on key cybersecurity topics that must be understood, they only promote greater
emphasis on a subset of topics. For example, NICE covers a wide range of key topics but gaps exist
such as with topics related to cyber-physical systems and human factors, and the NCSC Certified
Master's Program guidelines do not put much emphasis on important topics such as software security, but
in contrast with others place emphasis on attacks and defences. The CyBOK project, developed by the
NCSC, codifies foundational knowledge into 21 knowledge areas in 5 categories. It has been shown
that, in comparison with other knowledge frameworks, CyBOK covers a wide range of knowledge areas
and does not have gaps that are present with some other frameworks~\cite{hallett2018mirror}.

% Then talk about cybersecurity learning platforms and cards, highlighting some limitations of those
% approaches which will back up this work

Aside from knowledge frameworks, such as CyBOK, cybersecurity information and how it is perceived and
understood has also shown to be presented in other ways.
Thomas et al.~\cite{thomas2019educational} proposed the use of a collectible card game (CCG)
as a means of teaching cybersecurity to high school students, given the benefits of
prevalence culturally to all age groups (familiarity) and encouraging the understanding
of competitive strategy and mistake-making as a way of learning~\cite{turkay2012collectible}.
Anvik et al.~\cite{anvik2019program} proposed the use of a web-based card game for learning
programming and cybersecurity concepts, using simple vocabulary to create ubiquitous learning
experiences. Denning et al.~\cite{denning2013control} proposed the use of a tabletop card game,
Control-Alt-Hack, with the aim of providing awareness training for cybersecurity,
arguing that playing card games can provide a reachable foundation for providing digestible
cybersecurity information to large audiences. As well as card games, other gamified approaches
include the likes of Capture The Flag (CTF) activities, for example, which provide competitive
exercises for finding vulnerabilities in computer systems and applications and have shown to be
a valuable learning tool~\cite{trickel2017shell,cybokctf,swann2021open}. While these gamified
approaches show to be successful for different demographics and use cases, there are limitations.
For example, card game approaches such as Control-Alt-Hack~\cite{denning2013control} do not cover
a broad range of what has been identified by knowledge frameworks as key topics. Furthermore, the
use of a games format does have limitations with regard to perceptions of quality, given the nature
of modern computer games, for example, as well as some may perceiving learning bespoke game
mechanics as tedious~\cite{denning2014practical}. With regard to other approaches, such as CTF
activities, while they have shown to be a very successful learning approach, this assumes that
configurations are done properly and can be easily administrated as well as rewarding to participants.
As well as this, they also require some degree of knowledge in cybersecurity, as well as more specific
knowledge of computer systems (e.g. command-line utilities) and specific software in order to be able
to participate well~\cite{mcdaniel2016capture}.
